Asynchronous Reconfiguration with Byzantine Failures

Replicated services are inherently vulnerable to failures and security breaches. In a long-running system, it is, therefore, indispensable to maintain a reconfiguration mechanism that would replace faulty replicas with correct ones. An important challenge is to enable reconfiguration without affecting the availability and consistency of the replicated data: the clients should be able to get correct service even when the set of service replicas is being updated. In this paper, we address the problem of reconfiguration in the presence of Byzantine failures: faulty replicas or clients may arbitrarily deviate from their expected behavior. We describe a generic technique for building asynchronous and Byzantine fault-tolerant reconfigurable objects: clients can manipulate the object data and issue reconfiguration calls without reaching consensus on the current configuration. With the help of forward-secure digital signatures, our solution makes sure that superseded and possibly compromised configurations are harmless, that slow clients cannot be fooled into reading stale data, and that Byzantine clients cannot cause a denial of service by flooding the system with reconfiguration requests. Our approach is modular and based on dynamic Byzantine lattice agreement abstraction, and we discuss how to extend it to enable Byzantine fault-tolerant implementations of a large class of reconfigurable replicated services.

==> algorithms/dbla-client.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CLIENT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{breakablealgorithm*}
    % \caption{{\DBLA}: code for client $p$ (part 1)}
    % \labelalg{dbla-client-1}

    \caption{{\DBLA}: code for client $p$}
    \labelalg{dbla-client}

  \BeginAlgorithmic
    \Parameters
      \State Lattice of configurations $\Conf$ and the initial configuration $\Cinit$
      \State The object lattice $\Lat$ and the initial value $\Vinit$
      \State Boolean functions $\fVerifyHistory(h, \sigma)$ and $\fVerifyInputValue(v, \sigma)$
    \EndParameters

    \Globals
      \State $\ihistory \subseteq \Conf$, initially $\{ \Cinit \}$                                        \Comment{local history of this process}
      \State $\Sigmahistory \in \Sigma$, initially $\bot$                                                 \Comment{proof for the local history}
      \State $\icurrentValues \subseteq \Lat \times \Sigma$, initially $\{ \Tupple{\Vinit, \bot} \}$      \Comment{known verifiable input values with proofs}
      \State $\istatus \in \{ \iinactive, \iproposing, \iconfirming \}$, initially $\iinactive$
      \State $\iseqNumber \in \mathbb{Z}$, initially $0$        \Comment{used to match requests with responses}
      \State $\iacks_1$, initially $\emptyset$                  \Comment{a set of pairs of form $\Tupple{\iprocessId, \isignature}$}
      \State $\iacks_2$, initially $\emptyset$                  \Comment{a set of pairs of form $\Tupple{\iprocessId, \isignature}$}
    \EndGlobals

    \AuxiliaryFunctions
      \State $\fMaxElement(h)$ \Comment{returns the {\thighest} configuration in history $h$}
      \State $\fContainsQuorum(\iacks, C)$ \Comment{returns $\iTrue$ iff ${\exists} Q \in \iquorums(C) \suchThat {\forall} r \in Q: \Tupple{r, *} \in \iacks$}
      \State $\fJoinAll(\ivs)$ \Comment{returns the lattice join of all elements in $\ivs$}
      \State $\fVerifyValues(\ivs)$ \Comment{returns $\iTrue$ iff $\forall \Tupple{v, \sigma} \in \ivs: \fVerifyInputValue(v, \sigma)$}
      \State $\fFSVerify(m, r, s, t)$ \Comment{verifies forward-secure signature (see Section~\ref{sec:system-model})}
    \EndAuxiliaryFunctions

    \algspace
    \Operation{$\fPropose$}{$v$, $\sigma$} \labelline{propose}
      \State $\fRefine(\{ \Tupple{v, \sigma} \})$ \labelline{propose-refine}
      \State \WaitFor $\fContainsQuorum(\iacks_2, \fMaxElement(\ihistory))$ \labelline{propose-wait}
      \State $\istatus \gets \iinactive$ \labelline{propose-after-wait}
      \State let $\sigma = \Tupple{\icurrentValues, \ihistory, \Sigmahistory, \iacks_1, \iacks_2}$                      \labelline{propose-make-proof}
      \State \Return $\Tupple{\fJoinAll(\icurrentValues), \sigma}$                                                      \labelline{propose-return}
    \EndOperation

    \algspace
    \Operation{$\fUpdateHistory$}{$h$, $\sigma$}                                                                        \labelline{update-history}
      \State \RBBroadcast{$\mNewHistory$, $h$, $\sigma$}
    \EndOperation
    
    \Function{$\fVerifyOutputValue$}{$v$, $\sigma$} \labelline{verify-output-value}
      \If {$\sigma = \bot$} \Return $v = \Vinit$ \EndIf
      %
      \State let $\Tupple{\ivalues, h, \sigma_h, \iproposeAcks, \iconfirmAcks} = \sigma$ \labelline{verify-output-value-unpack}
      \State let $C = \fMaxElement(h)$
      %
      \State \Return $\fJoinAll(\ivalues) = v \land \fVerifyHistory(h, \sigma_h)$ \labelline{verify-output-value-verify-history}
          $\tlaStyleLand \fContainsQuorum(\iproposeAcks, C) \land \fContainsQuorum(\iconfirmAcks, C)$
          $\tlaStyleLand \forall\; \Tupple{r, s} \in \iproposeAcks: \fFSVerify(\Tupple{\mProposeResp, \ivalues}, r, s, \iheight(C))$
          $\tlaStyleLand \forall\; \Tupple{r, s} \in \iconfirmAcks: \fFSVerify(\Tupple{\mConfirmResp, \iproposeAcks}, r, s, \iheight(C))$ \labelline{verify-output-value-end}
    \EndFunction
    
%   \EndAlgorithmic
% \end{algorithm*}

% \begin{algorithm*}
%   \caption{{\DBLA}: code for client $p$ (part 2)}
%   \labelalg{dbla-client-2}
  
%   \BeginAlgorithmic

    \algspace
    \Procedure{$\fRefine$}{$\ivalues$}                                                                                  \labelline{refine}
      \State $\iacks_1 \gets \emptyset$; $\iacks_2 \gets \emptyset$
      \State $\icurrentValues \gets \icurrentValues \cup \ivalues$                                                      \labelline{refine-current-values}
      \State $\iseqNumber \gets \iseqNumber + 1$
      \State $\istatus \gets \iproposing$
      \State let $C = \fMaxElement(\ihistory)$
      \State \Send{$\mPropose$, $\icurrentValues$, $\iseqNumber$, $C$}{$\ireplicas(C)$}                                 \labelline{refine-send-message}
                                                                                                                        \labelline{refine-end}
    \EndProcedure

    \algspace
    \Upon{$\fContainsQuorum(\iacks_1, \fMaxElement(\ihistory))$}                                                        \labelline{upon-acks-collected}
      \State $\istatus \gets \iconfirming$
      \State let $C = \fMaxElement(\ihistory)$
      \State \Send{$\mConfirm$, $\iacks_1$, $\iseqNumber$, $C$}{$\ireplicas(C)$}                                        \labelline{upon-acks-collected-send-confirm}
    \EndHandler

    \algspace
    \UponReceive{$\mProposeResp$, $\ivalues$, $\isignature$, $\isn$}{replica $r$}                                       \labelline{upon-propose-resp}
      \State let $\isigValid = \fFSVerify(\Tupple{\mProposeResp, \ivalues}, r, \isignature, \iheight(\fMaxElement(\ihistory)))$
      \If {$\istatus = \iproposing \land \isn = \iseqNumber \land \isigValid$} \labelline{upon-propose-resp-check}
        \If {$\ivalues \nsubseteq \icurrentValues \land \fVerifyValues(\ivalues \setminus \icurrentValues)$} $\fRefine(\ivalues)$ \labelline{upon-propose-resp-refine}
        \ElsIf {$\ivalues = \icurrentValues$} $\iacks_1 \gets \iacks_1 \cup \{ \Tupple{r, \isignature} \}$              \labelline{upon-propose-resp-ack}
        \EndIf
      \EndIf                                                                                                            \labelline{upon-propose-resp-end}
    \EndHandler

    \algspace
    \UponReceive{$\mConfirmResp$, $\isignature$, $\isn$}{replica $r$}
      \State let $\isigValid = \fFSVerify(\Tupple{\mConfirmResp, \iacks_1}, r, \isignature, \iheight(\fMaxElement(\ihistory)))$
      \If {$\istatus = \iconfirming \land \isn = \iseqNumber \land \isigValid$}
        $\iacks_2 \gets \iacks_2 \cup \{ \Tupple{r, \isignature} \}$
      \EndIf
    \EndHandler

    \algspace
    \UponRBDeliver{$\mNewHistory$, $h$, $\sigma$}{any sender}                                                           \labelline{new-history}
      \If {$\fVerifyHistory(h, \sigma) \land \ihistory \subset h$}                                                      \labelline{new-history-verify}
        \State $\ihistory \gets h$; $\Sigmahistory \gets \sigma$                                                        \labelline{history-update}
        % \State \textbf{trigger} upcall $\fNewHistory(h)$
        \If {$\istatus \in \{ \iproposing, \iconfirming \}$} $\fRefine(\emptyset)$ \EndIf                               \labelline{new-history-refine}
      \EndIf
    \EndHandler
  \EndAlgorithmic
\end{breakablealgorithm*}



==> algorithms/dbla-full.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% CLIENT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{breakablealgorithm*}
    % \caption{{\DBLA}: code for client $p$ (part 1)}
    % \labelalg{dbla-client-1}

    \caption{{\DBLA}: code for client $p$}
    \labelalg{dbla-client}

  \BeginAlgorithmic
    \Parameters
      \State Lattice of configurations $\Conf$ and the initial configuration $\Cinit$
      \State The object lattice $\Lat$ and the initial value $\Vinit$
      \State Boolean functions $\fVerifyHistory(h, \sigma)$ and $\fVerifyInputValue(v, \sigma)$
    \EndParameters

    \Globals
      \State $\ihistory \subseteq \Conf$, initially $\{ \Cinit \}$                                        \Comment{local history of this process}
      \State $\Sigmahistory \in \Sigma$, initially $\bot$                                                 \Comment{proof for the local history}
      \State $\icurrentValues \subseteq \Lat \times \Sigma$, initially $\{ \Tupple{\Vinit, \bot} \}$      \Comment{known verifiable input values with proofs}
      \State $\istatus \in \{ \iinactive, \iproposing, \iconfirming \}$, initially $\iinactive$
      \State $\iseqNumber \in \mathbb{Z}$, initially $0$        \Comment{used to match requests with responses}
      \State $\iacks_1$, initially $\emptyset$                  \Comment{a set of pairs of form $\Tupple{\iprocessId, \isignature}$}
      \State $\iacks_2$, initially $\emptyset$                  \Comment{a set of pairs of form $\Tupple{\iprocessId, \isignature}$}
    \EndGlobals

    \AuxiliaryFunctions
      \State $\fMaxElement(h)$ \Comment{returns the {\thighest} configuration in history $h$}
      \State $\fContainsQuorum(\iacks, C)$ \Comment{returns $\iTrue$ iff ${\exists} Q \in \iquorums(C) \suchThat {\forall} r \in Q: \Tupple{r, *} \in \iacks$}
      \State $\fJoinAll(\ivs)$ \Comment{returns the lattice join of all elements in $\ivs$}
      \State $\fVerifyValues(\ivs)$ \Comment{returns $\iTrue$ iff $\forall \Tupple{v, \sigma} \in \ivs: \fVerifyInputValue(v, \sigma)$}
      \State $\fFSVerify(m, r, s, t)$ \Comment{verifies forward-secure signature (see Section~\ref{sec:system-model})}
    \EndAuxiliaryFunctions

    \algspace
    \Operation{$\fPropose$}{$v$, $\sigma$} \labelline{propose}
      \State $\fRefine(\{ \Tupple{v, \sigma} \})$ \labelline{propose-refine}
      \State \WaitFor $\fContainsQuorum(\iacks_2, \fMaxElement(\ihistory))$ \labelline{propose-wait}
      \State $\istatus \gets \iinactive$ \labelline{propose-after-wait}
      \State let $\sigma = \Tupple{\icurrentValues, \ihistory, \Sigmahistory, \iacks_1, \iacks_2}$                      \labelline{propose-make-proof}
      \State \Return $\Tupple{\fJoinAll(\icurrentValues), \sigma}$                                                      \labelline{propose-return}
    \EndOperation

    \algspace
    \Operation{$\fUpdateHistory$}{$h$, $\sigma$}                                                                        \labelline{update-history}
      \State \RBBroadcast{$\mNewHistory$, $h$, $\sigma$}
    \EndOperation
    
    \Function{$\fVerifyOutputValue$}{$v$, $\sigma$} \labelline{verify-output-value}
      \If {$\sigma = \bot$} \Return $v = \Vinit$ \EndIf
      %
      \State let $\Tupple{\ivalues, h, \sigma_h, \iproposeAcks, \iconfirmAcks} = \sigma$ \labelline{verify-output-value-unpack}
      \State let $C = \fMaxElement(h)$
      %
      \State \Return $\fJoinAll(\ivalues) = v \land \fVerifyHistory(h, \sigma_h)$ \labelline{verify-output-value-verify-history}
          $\tlaStyleLand \fContainsQuorum(\iproposeAcks, C) \land \fContainsQuorum(\iconfirmAcks, C)$
          $\tlaStyleLand \forall\; \Tupple{r, s} \in \iproposeAcks: \fFSVerify(\Tupple{\mProposeResp, \ivalues}, r, s, \iheight(C))$
          $\tlaStyleLand \forall\; \Tupple{r, s} \in \iconfirmAcks: \fFSVerify(\Tupple{\mConfirmResp, \iproposeAcks}, r, s, \iheight(C))$ \labelline{verify-output-value-end}
    \EndFunction
    
%   \EndAlgorithmic
% \end{algorithm*}

% \begin{algorithm*}
%   \caption{{\DBLA}: code for client $p$ (part 2)}
%   \labelalg{dbla-client-2}
  
%   \BeginAlgorithmic

    \algspace
    \Procedure{$\fRefine$}{$\ivalues$}                                                                                  \labelline{refine}
      \State $\iacks_1 \gets \emptyset$; $\iacks_2 \gets \emptyset$
      \State $\icurrentValues \gets \icurrentValues \cup \ivalues$                                                      \labelline{refine-current-values}
      \State $\iseqNumber \gets \iseqNumber + 1$
      \State $\istatus \gets \iproposing$
      \State let $C = \fMaxElement(\ihistory)$
      \State \Send{$\mPropose$, $\icurrentValues$, $\iseqNumber$, $C$}{$\ireplicas(C)$}                                 \labelline{refine-send-message}
                                                                                                                        \labelline{refine-end}
    \EndProcedure

    \algspace
    \Upon{$\fContainsQuorum(\iacks_1, \fMaxElement(\ihistory))$}                                                        \labelline{upon-acks-collected}
      \State $\istatus \gets \iconfirming$
      \State let $C = \fMaxElement(\ihistory)$
      \State \Send{$\mConfirm$, $\iacks_1$, $\iseqNumber$, $C$}{$\ireplicas(C)$}                                        \labelline{upon-acks-collected-send-confirm}
    \EndHandler

    \algspace
    \UponReceive{$\mProposeResp$, $\ivalues$, $\isignature$, $\isn$}{replica $r$}                                       \labelline{upon-propose-resp}
      \State let $\isigValid = \fFSVerify(\Tupple{\mProposeResp, \ivalues}, r, \isignature, \iheight(\fMaxElement(\ihistory)))$
      \If {$\istatus = \iproposing \land \isn = \iseqNumber \land \isigValid$} \labelline{upon-propose-resp-check}
        \If {$\ivalues \nsubseteq \icurrentValues \land \fVerifyValues(\ivalues \setminus \icurrentValues)$} $\fRefine(\ivalues)$ \labelline{upon-propose-resp-refine}
        \ElsIf {$\ivalues = \icurrentValues$} $\iacks_1 \gets \iacks_1 \cup \{ \Tupple{r, \isignature} \}$              \labelline{upon-propose-resp-ack}
        \EndIf
      \EndIf                                                                                                            \labelline{upon-propose-resp-end}
    \EndHandler

    \algspace
    \UponReceive{$\mConfirmResp$, $\isignature$, $\isn$}{replica $r$}
      \State let $\isigValid = \fFSVerify(\Tupple{\mConfirmResp, \iacks_1}, r, \isignature, \iheight(\fMaxElement(\ihistory)))$
      \If {$\istatus = \iconfirming \land \isn = \iseqNumber \land \isigValid$}
        $\iacks_2 \gets \iacks_2 \cup \{ \Tupple{r, \isignature} \}$
      \EndIf
    \EndHandler

    \algspace
    \UponRBDeliver{$\mNewHistory$, $h$, $\sigma$}{any sender}                                                           \labelline{new-history}
      \If {$\fVerifyHistory(h, \sigma) \land \ihistory \subset h$}                                                      \labelline{new-history-verify}
        \State $\ihistory \gets h$; $\Sigmahistory \gets \sigma$                                                        \labelline{history-update}
        % \State \textbf{trigger} upcall $\fNewHistory(h)$
        \If {$\istatus \in \{ \iproposing, \iconfirming \}$} $\fRefine(\emptyset)$ \EndIf                               \labelline{new-history-refine}
      \EndIf
    \EndHandler
  \EndAlgorithmic
\end{breakablealgorithm*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% REPLICA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{breakablealgorithm*}
  \caption{{\DBLA}: code for replica $r$}
  \labelalg{dbla-replica}

  \BeginAlgorithmic
    \ParametersInline $\Conf$, $\Lat$, $\Cinit$, $\Vinit$, $\fVerifyHistory(h, \sigma)$, and $\fVerifyInputValue(v, \sigma)$ (see Algorithm~\lstref{dbla-client})

    % \algspace
    \Globals
      \State $\ihistory \subseteq \Conf$, initially $\{ \Cinit \}$                        \Comment{local history of this process}
      \State $\icurrentValues \subseteq \Lat \times \Sigma$, initially $\{ \Tupple{\Vinit, \bot} \}$    \Comment{known verifiable input values with proofs}
      \State $\Ccurr \in \Conf$, initially $\Cinit$                                       \Comment{current configuration}
      \State $\Cinst \in \Conf$, initially $\Cinit$                                       \Comment{installed configuration}
      \State $\iseqNumber \in \mathbb{Z}$, initially $0$                                  \Comment{used to match requests with responses}
    \EndGlobals

    % \algspace
    \AuxiliaryFunctions
      \State $\fMaxElement$, $\fContainsQuorum$, $\fJoinAll$, $\fVerifyValues$ (see Algorithm~\lstref{dbla-client}).
      \State $\fFSSign(\mathit{message}, \mathit{timestamp})$ \Comment{produces a forward-secure signature (see Section~\ref{sec:system-model})}
      \State $\fUpdateFSKeys(t)$ \Comment{updates the signing timestamp (see Section~\ref{sec:system-model})}
    \EndAuxiliaryFunctions

    \algspace
    \UponReceive{$\mPropose$, $\ivalues$, $\isn$, $C$}{client $c$}                                                      \labelline{upon-propose}
      \State \WaitFor $C = \Cinst \lor \fMaxElement(\ihistory) \not\sqsubseteq C$                                       \labelline{upon-propose-wait}
      \If {$C = \fMaxElement(\ihistory) \land \fVerifyValues(\ivalues \setminus \icurrentValues)$}
        \State $\icurrentValues \gets \icurrentValues \cup \ivalues$                                                    \labelline{upon-propose-cur-vals}
        \State let $\isignature = \fFSSign(\Tupple{\mProposeResp, \icurrentValues}, \iheight(C))$                       \labelline{upon-propose-sign}
        \State \Send{$\mProposeResp$, $\icurrentValues$, $\isignature$, $\isn$}{$c$}
      \Else{} ignore the message
      \EndIf                                                                                                            \labelline{upon-propose-end}
    \EndHandler

    \algspace
    \UponReceive{$\mConfirm$, $\iproposeAcks$, $\isn$, $C$}{client $c$}                                                 \labelline{upon-confirm}
      \State \WaitFor $C = \Cinst \lor \fMaxElement(\ihistory) \not\sqsubseteq C$                                       \labelline{upon-confirm-wait}
      \If {$C = \fMaxElement(\ihistory)$}
        \State let $\isignature = \fFSSign(\Tupple{\mConfirmResp, \iproposeAcks}, \iheight(C))$                         \labelline{upon-confirm-sign}
        \State \Send{$\mConfirmResp$, $\isignature$, $\isn$}{$c$}
      \Else{} ignore the message
      \EndIf
    \EndHandler

    \algspace
    \LineCommentx{State transfer}
    \Upon{$\Ccurr \neq \fMaxElement(\{ C \in \ihistory \mid r \in \ireplicas(C) \})$}                                    \labelline{state-transfer-begin}
      \State let $\Cnext = \fMaxElement(\{ C \in \ihistory \mid r \in \ireplicas(C) \})$                                 \labelline{state-transfer-first-line}
      \State let $S = \{ C \in \ihistory \mid \Ccurr \sqsubseteq C \sqsubset \Cnext \}$                                  \labelline{state-transfer-speculation}
      \State $\iseqNumber \gets \iseqNumber + 1$
      \ForEach {$C \in S$}                                                                                              \labelline{state-transfer-for-begin}
        \State \Send{$\mUpdateRead$, $\iseqNumber$, $C$}{$\ireplicas(C)$}                                               \labelline{state-transfer-update-read}
        \State \WaitFor ($C \sqsubset \Ccurr$) $\lor$ (responses from any $Q \in \iquorums(C)$ with s.n. $\iseqNumber$) \labelline{state-transfer-wait}
      \EndFor                                                                                                           \labelline{state-transfer-for-end}
      \If {$\Ccurr \sqsubset \Cnext$}
        \State $\Ccurr \gets \Cnext$                                                                                    \labelline{state-transfer-ccurr-set}
        \State \URBBroadcastIn{$\mUpdateComplete$}{$\Cnext$}                                                            \labelline{state-transfer-broadcast}
      \EndIf                                                                                                            \labelline{state-transfer-end}
    \EndHandler

    \algspace
    \UponRBDeliver{$\mNewHistory$, $h$, $\sigma$}{any sender}                                                           \labelline{new-history}
      \If {$\fVerifyHistory(h, \sigma) \land \ihistory \subset h$}                                                      \labelline{new-history-verify}
        \State $\ihistory \gets h$
        % \State \textbf{trigger} upcall $\fNewHistory(h)$
        \State $\fUpdateFSKeys(\iheight(\fMaxElement(\ihistory)))$                                                      \labelline{new-history-update-fs-keys}
      \EndIf                                                                                                            \labelline{new-history-end}
    \EndHandler

    \algspace
    \UponReceive{$\mUpdateRead$, $\isn$, $C$}{replica $r'$}                                                             \labelline{upon-update-read}
      \State \WaitFor $C \sqsubset \fMaxElement(\ihistory)$ \Comment{only reply after $\fUpdateFSKeys$}                 \labelline{upon-update-read-wait}
      \State \Send{$\mUpdateReadResp$, $\icurrentValues$, $\isn$}{$r'$}                                                 \labelline{upon-update-read-send-resp}
    \EndHandler

    \algspace
    \UponReceive{$\mUpdateReadResp$, $\ivalues$, $\isn$}{replica $r'$}
      \If {$\fVerifyValues(\ivalues \setminus \icurrentValues)$} $\icurrentValues \gets \icurrentValues \cup \ivalues$ \EndIf
    \EndHandler

    \algspace
    \UponURBDeliverIn{$\mUpdateComplete$}{$C$}{quorum $Q \in \iquorums(C)$}                                             \labelline{upon-update-complete}
      \State \WaitFor $C \in \ihistory$                                                                                 \labelline{upon-update-complete-wait}
      \If {$\Cinst \sqsubset C$}                                                                                        \labelline{upon-update-complete-if}
        \If {$\Ccurr \sqsubset C$} $\Ccurr \gets C$ \EndIf                                                              \labelline{upon-update-complete-ccurr-set}
        \State $\Cinst \gets C$                                                                                         \labelline{upon-update-complete-cinst-set}
        \State \textbf{trigger} upcall $\fInstalledConfig(C)$                                                           \labelline{upon-update-complete-upcall}
        \If {$r \notin \ireplicas(C)$} halt \EndIf
      \EndIf                                                                                                            \labelline{upon-update-complete-end}
    \EndHandler
  \EndAlgorithmic
\end{breakablealgorithm*}


==> algorithms/dbla-replica.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% REPLICA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{breakablealgorithm*}
  \caption{{\DBLA}: code for replica $r$}
  \labelalg{dbla-replica}

  \BeginAlgorithmic
    \ParametersInline $\Conf$, $\Lat$, $\Cinit$, $\Vinit$, $\fVerifyHistory(h, \sigma)$, and $\fVerifyInputValue(v, \sigma)$ (see Algorithm~\lstref{dbla-client})

    \algspace
    \Globals
      \State $\ihistory \subseteq \Conf$, initially $\{ \Cinit \}$                        \Comment{local history of this process}
      \State $\icurrentValues \subseteq \Lat \times \Sigma$, initially $\{ \Tupple{\Vinit, \bot} \}$    \Comment{known verifiable input values with proofs}
      \State $\Ccurr \in \Conf$, initially $\Cinit$                                       \Comment{current configuration}
      \State $\Cinst \in \Conf$, initially $\Cinit$                                       \Comment{installed configuration}
      \State $\iseqNumber \in \mathbb{Z}$, initially $0$                                  \Comment{used to match requests with responses}
    \EndGlobals

    \algspace
    \AuxiliaryFunctions
      \State $\fMaxElement$, $\fContainsQuorum$, $\fJoinAll$, $\fVerifyValues$ (see Algorithm~\lstref{dbla-client}).
      \State $\fFSSign(\mathit{message}, \mathit{timestamp})$ \Comment{produces a forward-secure signature (see Section~\ref{sec:system-model})}
      \State $\fUpdateFSKeys(t)$ \Comment{updates the signing timestamp (see Section~\ref{sec:system-model})}
    \EndAuxiliaryFunctions

    \algspace
    \UponReceive{$\mPropose$, $\ivalues$, $\isn$, $C$}{client $c$}                                                      \labelline{upon-propose}
      \State \WaitFor $C = \Cinst \lor \fMaxElement(\ihistory) \not\sqsubseteq C$                                       \labelline{upon-propose-wait}
      \If {$C = \fMaxElement(\ihistory) \land \fVerifyValues(\ivalues \setminus \icurrentValues)$}
        \State $\icurrentValues \gets \icurrentValues \cup \ivalues$                                                    \labelline{upon-propose-cur-vals}
        \State let $\isignature = \fFSSign(\Tupple{\mProposeResp, \icurrentValues}, \iheight(C))$                       \labelline{upon-propose-sign}
        \State \Send{$\mProposeResp$, $\icurrentValues$, $\isignature$, $\isn$}{$c$}
      \Else{} ignore the message
      \EndIf                                                                                                            \labelline{upon-propose-end}
    \EndHandler

    \algspace
    \UponReceive{$\mConfirm$, $\iproposeAcks$, $\isn$, $C$}{client $c$}                                                 \labelline{upon-confirm}
      \State \WaitFor $C = \Cinst \lor \fMaxElement(\ihistory) \not\sqsubseteq C$                                       \labelline{upon-confirm-wait}
      \If {$C = \fMaxElement(\ihistory)$}
        \State let $\isignature = \fFSSign(\Tupple{\mConfirmResp, \iproposeAcks}, \iheight(C))$                         \labelline{upon-confirm-sign}
        \State \Send{$\mConfirmResp$, $\isignature$, $\isn$}{$c$}
      \Else{} ignore the message
      \EndIf
    \EndHandler

    \algspace
    \LineCommentx{State transfer}
    \Upon{$\Ccurr \neq \fMaxElement(\{ C \in \ihistory \mid r \in \ireplicas(C) \})$}                                    \labelline{state-transfer-begin}
      \State let $\Cnext = \fMaxElement(\{ C \in \ihistory \mid r \in \ireplicas(C) \})$                                 \labelline{state-transfer-first-line}
      \State let $S = \{ C \in \ihistory \mid \Ccurr \sqsubseteq C \sqsubset \Cnext \}$                                  \labelline{state-transfer-speculation}
      \State $\iseqNumber \gets \iseqNumber + 1$
      \ForEach {$C \in S$}                                                                                              \labelline{state-transfer-for-begin}
        \State \Send{$\mUpdateRead$, $\iseqNumber$, $C$}{$\ireplicas(C)$}                                               \labelline{state-transfer-update-read}
        \State \WaitFor ($C \sqsubset \Ccurr$) $\lor$ (responses from any $Q \in \iquorums(C)$ with s.n. $\iseqNumber$) \labelline{state-transfer-wait}
      \EndFor                                                                                                           \labelline{state-transfer-for-end}
      \If {$\Ccurr \sqsubset \Cnext$}
        \State $\Ccurr \gets \Cnext$                                                                                    \labelline{state-transfer-ccurr-set}
        \State \URBBroadcastIn{$\mUpdateComplete$}{$\Cnext$}                                                            \labelline{state-transfer-broadcast}
      \EndIf                                                                                                            \labelline{state-transfer-end}
    \EndHandler

    \algspace
    \UponRBDeliver{$\mNewHistory$, $h$, $\sigma$}{any sender}                                                           \labelline{new-history}
      \If {$\fVerifyHistory(h, \sigma) \land \ihistory \subset h$}                                                      \labelline{new-history-verify}
        \State $\ihistory \gets h$
        % \State \textbf{trigger} upcall $\fNewHistory(h)$
        \State $\fUpdateFSKeys(\iheight(\fMaxElement(\ihistory)))$                                                      \labelline{new-history-update-fs-keys}
      \EndIf                                                                                                            \labelline{new-history-end}
    \EndHandler

    \algspace
    \UponReceive{$\mUpdateRead$, $\isn$, $C$}{replica $r'$}                                                             \labelline{upon-update-read}
      \State \WaitFor $C \sqsubset \fMaxElement(\ihistory)$ \Comment{only reply after $\fUpdateFSKeys$}                 \labelline{upon-update-read-wait}
      \State \Send{$\mUpdateReadResp$, $\icurrentValues$, $\isn$}{$r'$}                                                 \labelline{upon-update-read-send-resp}
    \EndHandler

    \algspace
    \UponReceive{$\mUpdateReadResp$, $\ivalues$, $\isn$}{replica $r'$}
      \If {$\fVerifyValues(\ivalues \setminus \icurrentValues)$} $\icurrentValues \gets \icurrentValues \cup \ivalues$ \EndIf
    \EndHandler

    \algspace
    \UponURBDeliverIn{$\mUpdateComplete$}{$C$}{quorum $Q \in \iquorums(C)$}                                             \labelline{upon-update-complete}
      \State \WaitFor $C \in \ihistory$                                                                                 \labelline{upon-update-complete-wait}
      \If {$\Cinst \sqsubset C$}                                                                                        \labelline{upon-update-complete-if}
        \If {$\Ccurr \sqsubset C$} $\Ccurr \gets C$ \EndIf                                                              \labelline{upon-update-complete-ccurr-set}
        \State $\Cinst \gets C$                                                                                         \labelline{upon-update-complete-cinst-set}
        \State \textbf{trigger} upcall $\fInstalledConfig(C)$                                                           \labelline{upon-update-complete-upcall}
        \If {$r \notin \ireplicas(C)$} halt \EndIf
      \EndIf                                                                                                            \labelline{upon-update-complete-end}
    \EndHandler
  \EndAlgorithmic
\end{breakablealgorithm*}


==> algorithms/dbla-state-transfer.tex <==
\begin{algorithm*}
  \caption{{\DBLA} state transfer, code for replica $r$}
  \labelalg{dbla-state-transfer}

  \BeginAlgorithmic
    % \UponRBDeliver{$\mNewHistory$, $h$, $\sigma$}{any sender}                                                           \labelline{new-history}
    %   \If {$\fVerifyHistory(h, \sigma) \land \ihistory \subset h$}                                                    \labelline{new-history-verify}
    %     \State $\ihistory \gets h$
    %     \State $\fUpdateFSKeys(\iheight(\fMaxElement(\ihistory)))$                                                    \labelline{new-history-update-fs-keys}
    %   \EndIf                                                                                                            \labelline{new-history-end}
    % \EndHandler

    \algspace
    \Upon{$\Ccurr \neq \fMaxElement(\{ C \in \ihistory \mid r \in \ireplicas(C) \})$}                                    \labelline{state-transfer-begin}
      \State let $\Cnext = \fMaxElement(\{ C \in \ihistory \mid r \in \ireplicas(C) \})$                                 \labelline{state-transfer-first-line}
      \State let $S = \{ C \in \ihistory \mid \Ccurr \sqsubseteq C \sqsubset \Cnext \}$                                  \labelline{state-transfer-speculation}
      \State $\iseqNumber \gets \iseqNumber + 1$
      \ForEach {$C \in S$}                                                                                              \labelline{state-transfer-for-begin}
        \State \Send{$\mUpdateRead$, $\iseqNumber$, $C$}{$\ireplicas(C)$}                                               \labelline{state-transfer-update-read}
        \State \WaitFor ($C \sqsubset \Ccurr$) $\lor$ (responses from any $Q \in \iquorums(C)$ with s.n. $\iseqNumber$) \labelline{state-transfer-wait}
      \EndFor                                                                                                           \labelline{state-transfer-for-end}
      \If {$\Ccurr \sqsubset \Cnext$}
        \State $\Ccurr \gets \Cnext$                                                                                    \labelline{state-transfer-ccurr-set}
        \State \URBBroadcastIn{$\mUpdateComplete$}{$\Cnext$}                                                            \labelline{state-transfer-broadcast}
      \EndIf                                                                                                            \labelline{state-transfer-end}
    \EndHandler

    \algspace
    \UponReceive{$\mUpdateRead$, $\isn$, $C$}{replica $r'$}                                                             \labelline{upon-update-read}
      \State \WaitFor $C \sqsubset \fMaxElement(\ihistory)$                                                             \labelline{upon-update-read-wait}
      \State \Send{$\mUpdateReadResp$, $\icurVals$, $\isn$}{$r'$}                                                       \labelline{upon-update-read-send-resp}
    \EndHandler

    \algspace
    \UponReceive{$\mUpdateReadResp$, $\ivalues$, $\isn$}{replica $r'$}
      \If {$\fVerifyValues(\ivalues \setminus \icurVals)$} $\icurVals \gets \icurVals \cup \ivalues$ \EndIf
    \EndHandler

    \algspace
    \UponURBDeliverIn{$\mUpdateComplete$}{$C$}{quorum $Q \in \iquorums(C)$}                                             \labelline{upon-update-complete}
      \State \WaitFor $C \in \ihistory$                                                                                 \labelline{upon-update-complete-wait}
      \If {$\Cinst \sqsubset C$}                                                                                        \labelline{upon-update-complete-if}
        \If {$\Ccurr \sqsubset C$} $\Ccurr \gets C$ \EndIf                                                              \labelline{upon-update-complete-ccurr-set}
        \State $\Cinst \gets C$                                                                                         \labelline{upon-update-complete-cinst-set}
        \State \textbf{trigger} upcall $\fInstalledConfig(C)$                                                           \labelline{upon-update-complete-upcall}
        \If {$r \notin \ireplicas(C)$} halt \EndIf
      \EndIf                                                                                                            \labelline{upon-update-complete-end}
    \EndHandler
  \EndAlgorithmic
\end{algorithm*}

==> figures/dbla-and-transform.tex <==
\begin{figure}
  \centering

  \begin{subfigure}{\linewidth}
    \centering
    % \raggedright
    \pdftex[\linewidth]{compiled-drawings/dbla-interface.pdf_tex}
    \caption{The interface of {\DBLA}.}
    \label{fig:dbla-interface}
  \end{subfigure}
  
  \begin{subfigure}{\linewidth}
    \centering
    % \raggedright
    \pdftex[\linewidth]{compiled-drawings/transform.pdf_tex}
    \caption{The dependencies in a {\reconfigurable} object.}
    \label{fig:transform}
  \end{subfigure}

  \caption{
    \textbf{(a):}
    %
    The interface of a {\DBLA} object.
    Parameters are depicted on the left side,
    operations and functions are on the right side,
    and upcalls are at the top.
    %
    The parts of the interface that are inherited from {\BLA} are depicted
    as \needsrev{solid} black arrows, while the parts of the interface that are inherited
    from the specification of a {\dynamic} object are depicted as dashed blue arrows.
    %
    ``$\mathrm{IV}$'', ``$\mathrm{OV}$'', and ``$\mathrm{Hist}$'' are abbreviations for
    ``$\mathrm{InputValue}$'', ``$\mathrm{OutputValue}$'', and ``$\mathrm{History}$'', respectively.
    %
    \textbf{(b):}
    The structure of dependencies in our implementation of a reconfigurable object.
    % $\fVIV$ and $\fVH$ stand for $\fVerifyInputValue$ and $\fVerifyHistory$ respectively.
    An arrow from an object $A$ to another object $B$ marked with $\fVIV$ (resp., $\fVH$)
    indicates that $A.\fVerifyInputValue$ (resp., $A.\fVerifyHistory$) is implemented using $B.\fVerifyOutputValue$.
    % indicates that $A$ uses $B.\fVerifyOutputValue$ to implement $A.\fVerifyInputValue$ (resp., $A.\fVerifyHistory$).
    %
    % All three {\dynamic} objects use $\iHistLA$ as the source of verifiable histories (including $\iHistLA$ itself).
    % Verifiable input values for $\iConfLA$ are the verifiable input configurations of the {\reconfigurable} object.
    % Verifiable input values for $\iHistLA$ are singleton sets of verifiable output values of $\iConfLA$.
    % Finally, verifiable input values for $\iDObj$ are the verifiable input values of the reconfigurable object.
  }
  \label{fig:dbla-and-transform}
\end{figure}


==> specs/transform-spec.tex <==

\begin{algorithm*}
    \caption{Reconfigurable object specification}
    \labelalg{transform-spec}
    
    \BeginAlgorithmic
        \Parameters
            \State Dynamic object $\iDObj$
            \State Boolean function $\fVerifyConf(C, \sigma)$
            \State All the parameters of $\iDObj$ except the function $\fVerifyHistory$ (including lattice of configurations $\Conf$ and the initial configuration $\Cinit \in \Conf$)
        \EndParameters
        
    %     \algspace
    %     \Interface
    %         \Operation{$\fPropose$}{$v$, $\sigma$} \EndOperation
    %         \Operation{$\fUpdateHistory$}{$h$, $\sigma$} \EndOperation
    %         \Function{$\fVerifyOutputValue$}{$v$, $\sigma$} \EndFunction
    %         \Upcall{$\fInstalledConfig$}{$C$} \EndUpcall
    %     \EndInterface
        
    %     \algspace
    %     \PropertiesInline
    %             {\pBLAValidity},
    %             {\pBLAVerifiability},
    %             {\pBLAInclusion},
    %             {\pBLAComparability},
    %             {\pBLALiveness},
    %             \\ \hspace{\algorithmicindent}
    %             {\pDynamicValidity},
    %             {\pDynamicLiveness},
    %             {\pInstallationLiveness}
    % \EndAlgorithmic
\end{algorithm*}

